TikZero: Zero-Shot Text-Guided Graphics Program Synthesis

Automatically synthesizing figures from text captions is a compelling capability. However, achieving high geometric precision and editability requires representing figures as graphics programs in languages like TikZ, and aligned training data (i.e., graphics programs with captions) remains scarce. Meanwhile, large amounts of unaligned graphics programs and captioned raster images are more readily available. We reconcile these disparate data sources by presenting TikZero, which decouples graphics program generation from text understanding by using image representations as an intermediary bridge. It enables independent training on graphics programs and captioned images and allows for zero-shot text-guided graphics program synthesis during inference. We show that our method substantially outperforms baselines that can only operate with caption-aligned graphics programs. Furthermore, when leveraging caption-aligned graphics programs as a complementary training signal, TikZero matches or exceeds the performance of much larger models, including commercial systems like GPT-4o. Our code, datasets, and select models are publicly available.

==> graphics/examples/evaluation/caption/0/caption.tex <==
An illustration of the reduction from densest $k$-subgraph to {{\sc u-rcp}}. On the left there is a simple undirected graph $G$ with a single edge. The $2$-reduced directed graph of $G$ is on the right. Each vertex of $G$ is replaced by $2\cdot2 = 4$ copies with a bidirectional edge connecting any two copies of the same vertex, and an outgoing edge from each copy to the single edge-vertex $e$.

==> graphics/examples/evaluation/caption/1/caption.tex <==
Domain of dependence: The closed trapezoidal region $\Omega_t$ used in the proof of {\sc proposition} \ref{prop: finite propagation speed}, shaded with darker yellow; the domain of dependence of point $(0,\ell)$ is $\Omega_t$ along with the top region shaded with lighter yellow.

==> graphics/examples/evaluation/caption/2/caption.tex <==
A sketch of iterating $f(x) = x-1/x$. Points bigger than 1 get sent to point in $[0,1]$ which then moves to a point $\leq -1$ which moves to $[-1,0]$ which is sent to a point $\geq 1$ and so on.


==> graphics/examples/evaluation/caption/3/caption.tex <==
A multiline diagram $D$ with $n=6$ columns and $s=5$ rows, with content $\lambda=(5,4,3,1,0,0)$ and bottom row $\rho^{(1)}(D)=(4,0,1,5,3,0)\in S_\lambda$. It has weight $\operatorname{w}(D)=\operatorname{w}_x(D) \operatorname{w}_t(D)=x_1^3 x_3^2 x_4^4 x_5^2 x_6^2\, t^2$.

